Polarization-encoded co-localization microscopy at cryogenic temperatures

Super-resolution localization microscopy is based on determining the positions of individual fluorescent markers in a sample. The major challenge in reaching an ever higher localization precision lies in the limited number of collected photons from single emitters. To tackle this issue, it has been shown that one can exploit the increased photostability at low temperatures, reaching localization precisions in the sub-nanometer range. Another crucial ingredient of single-molecule super-resolution imaging is the ability to activate individual emitter within a diffraction-limited spot. Here, we report on photoblinking behavior of organic dyes at low temperature and elaborate on the limitations of this ubiquitous phenomenon for selecting single molecules. We then show that recording the emission polarization not only provides access to the molecular orientation, but it also facilitates the assignment of photons to individual blinking molecules. Furthermore, we employ periodical modulation of the excitation polarization as a robust method to effectively switch fluorophores. We bench mark each approach by resolving two emitters on different DNA origami structures.

==> xx.tex <==


